Transparent and Scrutable Recommendations Using Natural Language User Profiles

Recent state-of-the-art recommender systems predominantly rely on either implicit or explicit feedback from users to suggest new items. While effective in recommending novel options, many recommender systems often use uninterpretable embeddings to represent user preferences. This lack of transparency not only limits user understanding of why certain items are suggested but also reduces the user's ability to scrutinize and modify their preferences, thereby affecting their ability to receive a list of preferred recommendations. Given the recent advances in Large Language Models (LLMs), we investigate how a properly crafted prompt can be used to summarize a user's preferences from past reviews and recommend items based only on language-based preferences. In particular, we study how LLMs can be prompted to generate a natural language (NL) user profile that holistically describe a user's preferences. These NL profiles can then be leveraged to fine-tune a LLM using only NL profiles to make transparent and scrutable recommendations. Furthermore, we validate the scrutability of our user profile-based recommender by investigating the impact on recommendation changes after editing NL user profiles. According to our evaluations of the model's rating prediction performance on two benchmarking rating prediction datasets, we observe that this novel approach maintains a performance level on par with established recommender systems in a warm-start setting. With a systematic analysis into the effect of updating user profiles and system prompts, we show the advantage of our approach in easier adjustment of user preferences and a greater autonomy over users' received recommendations.

==> sections/mitigate_bias.tex <==
In order to test the benefits of the scrutability of UPR, we experiment with modifying an NL profile to make the recommendations more `fair'. In this case, we define `fair' as an increased coverage of a target minority group. In particular, we experiment with making the recommendations for Amazon-MT more fair with regards to the director's gender, language of the movie, and the production country. We note that these \textit{sensitive attributes} are commonly chosen to study bias in recommender systems~\cite{ferraro2022Commonality}.

Since the Amazon-MT dataset does not contain the relevant metadata for each movie, we use The Movies Database (TMDB)\footnote{https://www.themoviedb.org} API to collect additional information about the movies, such as the movie's original language, the director's gender, the main country to movie was produced, and the year the movie was released. We filter out movies without our selected metadata, leaving us with about 66\% of the original data. Since the metadata is not encoded within the original model prompt, we add the metadata to the prompt during training and retrain UPR using the new dataset~\footnote{The full prompt used for training can be found in the repo.}.

% In particular, we use the following prompt during training: \\

% \noindent Rate the movie from 1 to 5 based on the user's profile and the information about the movie. The user's rating is influenced by the director's gender, the original language of the movie, genre of the movie, the production country, and the release year.

% \begin{itemize}
%     \item \textbf{User Profile:} \texttt{profile}
%     \item \textbf{Movie Title:} \texttt{Movie Title}
%     \item \textbf{Original Language:} \texttt{\{original\_language\}}
%     \item \textbf{Director's Gender:} \texttt{\{director\_gender\}}
%     \item \textbf{Production Country:} \texttt{\{production\_country\}}
%     \item \textbf{Release Year:} \texttt{\{release\_year\}}
%     \item \textbf{Rating:}
% \end{itemize}

Once the model is fine-tuned using the above prompt, we compare the performance of the original profile and modified profiles that push the model to be biased towards or against a given sensitive attribute (e.g. director gender, original language, and production country). In particular, for each sensitive attribute, we sample 100 movies that contain that sensitive attribute and 100 movies that do not contain the sensitive attribute. We then add a sentence to the beginning of the original NL profile that states that the user highly rates movies with the sensitive attribute or highly rates items with the non-sensitive attribute. We then run the model during inference time and calculate the coverage of the sensitive attributes for their top-k recommendations.

Overall, we found that there were no significant differences in recommendation between the two sets of attributes. We hypothesize that this occurred because 1) the model had not seen these types of preferences in the NL profile during training and 2) other preferences in the NL profile took precedent over these injected preferences. Thus, we added 2 in-context learning (ICL) examples to the prompt that demonstrated the desired behavior with regards to the sensitive attribute. ICL helps guide the model towards the desired output without having to retrain a model~\cite{brown2020language}.

As shown in Table~\ref{tab:fairness_coverage}, by scrutinizing the NL profile and adding ICL examples, we can easily make a model more fair. We hypothesize that if the model was trained with NL profiles that explicitly described preferences with regards to sensitive attributes, then the ICL examples would not be needed. Additionally, we hypothesize that the variance in coverage could be more pronounced for the original language of a film, as its language tends to be more readily apparent to an audience compared to aspects like the director's gender or the country of production. Nevertheless, we show the flexibility of using an NL-based approach to recommendations because we can change the recommendations to be more `fair' by simply adjusting the prompting without the need to retrain the model. In contrast, the user's interaction history would need to be significantly changed and the model would need to be retrained when using CF to give the  user `fair' recommendations.

\begin{table}[]
    \centering
    \begin{tabular}{llc}
        \toprule
         Category & Profile Sentence & Coverage@5 \\
         \hline
         Original Language & I highly rate movies with English as the main language. & 0.247 \\
         & I highly rate movies where the original language is not English. & 0.314 \\
         \hline
         Production Country & I highly rate movies produced in the USA. & 0.060 \\
         & I highly rate movies not produced in the USA. & 0.073 \\
         \hline
         Director Gender & I highly rate movies directed by males. &  0.281 \\
         & I highly rate movies directed by females. & 0.298 \\
         \bottomrule
    \end{tabular}
    \caption{Average Coverage for the top 5 recommendations across all users. The categories depict each of the three studied minority groups and the profile sentence is appended during inference time to biased the model towards or against a given sensitive attribute.}
    \label{tab:fairness_coverage}
\end{table}
% \begin{table}
% \centering
%   \caption{RMSE on selected criteria for Sensitive and Non-Sensitive}
%   \label{tab:bias}
%   \begin{tabular}{lcc|cc}
%     \toprule
%     Model & English & Non-English & Male Dir. & Non-male Dir. \\
%     \midrule
%     % MostPop
%     UserKNN & 0.961 & 0.940 & 0.958 & 0.986 \\
%     Item-KNN & 1.037 & 0.975 & 1.031 & 1.071 \\
%     MF & 0.924 & 0.905 & 0.922 & 0.945 \\
%     \midrule
%     PETER & 0.919 & 0.895 & 0.916 & 0.943 \\
%     PEPLER & 0.919 & 0.900 & 0.916 & 0.936 \\
%     \midrule
%     UPR & 0.940 & 0.917 & 0.937 & 0.969 \\
% \end{tabular}
% \end{table}

